Differentiable Grey-box Modelling of Phaser Effects using Frame-based Spectral Processing

Machine learning approaches to modelling analog audio effects have seen intensive investigation in recent years, particularly in the context of non-linear time-invariant effects such as guitar amplifiers. For modulation effects such as phasers, however, new challenges emerge due to the presence of the low-frequency oscillator which controls the slowly time-varying nature of the effect. Existing approaches have either required foreknowledge of this control signal, or have been non-causal in implementation. This work presents a differentiable digital signal processing approach to modelling phaser effects in which the underlying control signal and time-varying spectral response of the effect are jointly learned. The proposed model processes audio in short frames to implement a time-varying filter in the frequency domain, with a transfer function based on typical analog phaser circuit topology. We show that the model can be trained to emulate an analog reference device, while retaining interpretable and adjustable parameters. The frame duration is an important hyper-parameter of the proposed model, so an investigation was carried out into its effect on model accuracy. The optimal frame length depends on both the rate and transient decay-time of the target effect, but the frame length can be altered at inference time without a significant change in accuracy.

==> unused.tex <==

If the model is optimized using gradient descent, then this is approach is also known as differentiable DSP \cite{Engel2020}. Recently, DDSP approaches have been used to model distortion pedals \cite{Nercessian2021, Kuznetsov2020, Esqueda2021, Parker2019} and dynamic range compression \cite{Wright2022}.

Examples of this in VA modelling include Weiner-Hammerstein models for guitar amplifier emulation [], differentiable state-space models \cite{Esqueda2021} and differentiable DSP models for dynamic range compression \cite{Wright2022}.



Virtual analog modelling is an active area of research which seeks to accurately emulate these such devices using digital signal processing (DSP).The various approaches can be categorised into white-box, black-box and grey-box modelling. White-box modelling involves electrical analysis of the circuitry to derive the underlying physical equations of the device, then usually solving these numerically through methods such as state-space solvers, wave digital filters or port-Hamiltonian methods. 

Black-box modelling, in contrast, involves optimizing a generic model based on measurements of the reference device. Recent work has shown that neural networks can be effectively trained to act as perceptually convincing models of non-linear audio effects. Examples include the use of recurrent neural networks (RNNs) and temporal convolutional networks (TCNs) for guitar amplifier emulation \cite{Damskaag2018, Wright2019_RNN, Wright2020, Wright2021, Wright2022} and TCNs for dynamic range compression \cite{Steinmetz2021, Comunita2022}. 


Grey-box modelling, in general, combines aspects of both above approaches: typically using some domain knowledge to construct a model which is then optimized on measured data.  Examples of this in VA modelling include Weiner-Hammerstein models for guitar amplifier emulation [], differentiable state-space models \cite{Esqueda2021} and differentiable DSP models for dynamic range compression \cite{Wright2022}. 

Kiiski et al. \cite{Kiiski2016} used a grey-box approach to model a phaser device, in which visual inspection of spectral responses from a target device were used to infer the control  parameters for a digital phaser model. It was reported that the model did not perform well when modelling a phaser with a feedback loop []\cite{Kiiski2016}.
